Algorithms and Certificates for Boolean CSP Refutation: "Smoothed is no harder than Random"

We present an algorithm for strongly refuting smoothed instances of all Boolean CSPs. The smoothed model is a hybrid between worst and average-case input models, where the input is an arbitrary instance of the CSP with only the negation patterns of the literals re-randomized with some small probability. For an $n$-variable smoothed instance of a $k$-arity CSP, our algorithm runs in $n^{O(\ell)}$ time, and succeeds with high probability in bounding the optimum fraction of satisfiable constraints away from $1$, provided that the number of constraints is at least $\tilde{O}(n) (\frac{n}{\ell})^{\frac{k}{2} - 1}$. This matches, up to polylogarithmic factors in $n$, the trade-off between running time and the number of constraints of the state-of-the-art algorithms for refuting fully random instances of CSPs [RRS17]. We also make a surprising new connection between our algorithm and even covers in hypergraphs, which we use to positively resolve Feige's 2008 conjecture, an extremal combinatorics conjecture on the existence of even covers in sufficiently dense hypergraphs that generalizes the well-known Moore bound for the girth of graphs. As a corollary, we show that polynomial-size refutation witnesses exist for arbitrary smoothed CSP instances with number of constraints a polynomial factor below the "spectral threshold" of $n^{k/2}$, extending the celebrated result for random 3-SAT of Feige, Kim and Ofek [FKO06].

==> even-ref.tex <==

%!TEX root = main.tex
\ignore[old proof for even]{
\section{Refuting Regular Partitioned Polynomials for even $k$} 
In this section, we prove \cref{thm:partitioned-poly-refute-even}, restated below. 

\partitionedpolyrefuteeven*

Our proof follows a similar path as the one for the case when $k$ is odd with a crucial difference in the choice of the \kikuchi matrix. We present the proof in full details even though we adopt the same general scheme as in the previous section. Crucially, and in contrast to prior works, we need to apply the ``Cauchy-Schwarz trick'' even in the case when $k$ is even in order to handle the $p$-heavy partitioned polynomials. When $p =n$, this argument can be greatly simplified, but our decomposition from Lemma~\ref{lem:hypergraph-decomposition} results in instances where $p\gg n$ and thus the generalization to arbitrarily large $p$ is necessary for us. 


\begin{lemma}[Cauchy-Schwarz trick]
\label{lem:cauchy-schwarz-trick-even}
Let $k$ be an even integer. Let $\psi$ be a $p$-heavy partitioned homogeneous multilinear degree $k$ polynomial in $y=\{y_u\}_{u \leq p} \cup x=\{x_j\}_{j \leq n}$ described by a collection $\cH_u \subseteq {{[n]} \choose {k-1}}$, a collection of distinct $(k-1)$-tuples for every $u \leq p$ such that $\sum_{u \leq p} |\cH_u| = m \geq 4p/\epsilon^2$ and coefficients $\{b_{u,C}\}_{C \in \cH}$:
\[
\psi(y,x) = \frac{1}{m}\sum_{u \leq p} y_u \sum_{C \in \cH_u} b_{u,C} x_C\mper
\]

Then, for the $2(k-1)$ degree polynomial $f(x)$ defined by:
\begin{equation} \label{eq:poly-after-C-S}
 f(x) =\frac{p}{m^2} \sum_{u = 1}^p \sum_{C \ne C' \in \cH_u} b_{u,C} b_{u,C'} x_C x_{C'}\mcom
\end{equation} 
it holds that: $\val(\psi)^2 \leq \val(f) + \frac{\epsilon^2}{4}$.% and $\sosval_d(f) + O(\eps^2) \geq \sosval_d(\psi)^2$ for all $d \geq 2k$.
\end{lemma}
\begin{proof}
\begin{align*}
\psi^2(y,x) &= \Paren{\frac{1}{m} \sum_{u \leq p} y_u \sum_{C \in \cH_u} b_{u,C} x_C}^2 \leq \frac{1}{m^2} \Paren{\sum_{u \leq p} y_u^2} \Paren{ \sum_{u \leq p} \Paren{\sum_{C \in \cH_u} b_{u,C} x_C}^2}\\
&\leq \frac{p}{m^2}  \cdot \sum_{u \leq p} \sum_{C \in \cH_u} b_{u,C}^2 x_C^2 + \frac{p}{m^2}  \sum_{u \leq p } \sum_{C,C' \in \cH_u, C \neq C'} b_{u,C} b_{u,C'} x_C x_{C'}\\
&\leq \frac{p}{m} + \frac{p}{m^2} \sum_{u \leq p} \sum_{C,C' \in \cH_u, C \neq C'} b_{u,C} b_{u,C'} x_C x_{C'}\mper
\end{align*}
Here, the first inequality uses the Cauchy-Schwarz inequality. The second observes that $y_u^2 =1$ for every $u$. The third uses that $b_{u,C}^2 \leq 1$ and $x_C^2=1$. 

The first term on the RHS is at most $\frac{\epsilon^2}{4}$. Taking maximum of both sides now yields that $\val(\psi)^2 \leq \frac{\epsilon^2}{4} +  \val(f)$.
%For the second term, note that $\sum_{u\leq p} |\cH_u|^2 - \sum_{u \leq p} |\cH_u| \geq \frac{m^2}{p} - m \geq \frac{m^2}{2p}$ by Cauchy-Schwarz inequality. 


\end{proof}

We now present the variant of the \kikuchi matrix we will employ for even $k$ below. 

\begin{definition}[\kikuchi Matrix]
Let $k \in \N$ be even. Let $\ell = \ell(n)\in \N, \ell \geq k$. Let $\{\cH_u\}_{u \leq p}$ describe a collection of distinct $(k-1)$-tuples on $[n]$ for each $u \in [p]$. Let $\{b_{u,C}\}_{C \in \cH}$ be coefficients in $[-1,1]$ and let $f$ be the following associated polynomial of degree $2(k-1)$:
\[
f(x) =\frac{p}{m^2} \sum_{u = 1}^p \sum_{C \ne C' \in \cH_u} b_{u,C} b_{u,C'} x_C x_{C'}\mper
\]

For $N= {n \choose \ell}$, define the \kikuchi matrix of $f$, $A \in \R^{N^2 \times N^2}$ as follows. Associate the rows and columns of $A_f$ to pairs $(S_1, S_2), (T_1,T_2)$ such that each $S_i,T_i  \in {{[n]} \choose \ell}$ for $i = 1,2$. For any $C \subseteq [n]$ of size $k-1$, we define $S_1 \overset{C}{\rightarrow} T_1$ if $|C \cap S_1| = \frac{k}{2}$ and $|C \cap T_1| = \frac{k-2}{2}$, and these intersections contain disjoint parts of $C$.\peter{added this last part} Observe the asymmetry between the roles of $S_1$ and $T_1$ here. 

Define:
\begin{equation} \label{eq:kikuchi-matrix-def}
A^{(u)} ((S_1, S_2),(T_1, T_2)) = \frac{p}{m^2} \sum_{ \substack{(C, C') \in \cH_u \times \cH_u\\ S_1 \overset{C}{\rightarrow} T_1\\ T_2 \overset{C'}{\rightarrow} S_2}} b_{u,C} b_{u,C'} \mper
\end{equation}



Finally, set $A = \sum_{u \in [p]} A^{(u)}$. Note that $A$ is a symmetric matrix by construction. 

% If $k$ is even, let $N_k = {{p+n} \choose \ell} \cdot {{(k-2) n} \choose (k-2)\ell}$. 
% Define the \kikuchi matrix $A_f \in \R^{N_k \times N_k}$ as follows. 
% Associate the rows and columns of $A_f$ to pairs of sets $(S_1, S_2), (T_1, T_2)$ respectively where $|S_1|, |T_1| = \ell$ are subsets of the $p+n$ variables in $\{y_1, y_2, \ldots, y_p, x^{(1)}_1,x^{(1)}_2, \ldots, x^{(1)}_n\}$ and $|S_2|,|T_2|=(k-2)\ell$ are subsets of size $(k-2) \ell$ of the $(k-2)n$ variables in $\{x^{(i)}_j\}_{3 \leq i\leq k, j \leq n}$. For any such $S_1, S_2$ and $T_1, T_2$, we say that 

% Let $A \in \R^{N^2 \times N^2}$ be the matrix indexed by pairs $(S_1,S_2), (T_1, T_2) \in {[n] \choose \ell}^2$ defined by: 
% \[
% A( (S_1, S_2), (T_1, T_2)) = \frac{1}{\sqrt{\abs{\cH_u}}} \sum_{ \substack{C \neq C' \in \cH_u\\ S_1 \overset{C}{\leftrightarrow} T_1 \\ S_2 \overset{C'}{\leftrightarrow} T_2}} b_{u,C} b_{u,C'} \mper
% \]

\end{definition}

The \kikuchi matrix allows us to write $f$ as a quadratic form. % and thus, the $\infty \rightarrow 1$-norm $A$ upper-bounds $\val(f)$. Recall that $\Norm{A}_{\infty \rightarrow 1} = \frac{1}{N} \max_{y,z \in \on^N} y^{\top} Az$.  % leading to the following lemma that follows immediately from the definition of the \kikuchi matrix $A$. 
\begin{lemma}[f equals quadratic form \kikuchi matrix] \label{lem:symdiffmatrix}
For any $x \in \Fits^n$, let $x^{\star \ell} \in \Fits^{N^2}$ for $N= {n \choose \ell}$ be the vector where the $(S_1,S_2)$-th entry of $x^{\star \ell}$ is $\prod_{i \in S_1, j \in S_2} x_i x_j = x_{S_1} x_{S_2}$. Then, for $D={{k-1} \choose \frac{k}{2}} {{k-1} \choose \frac{k-2}{2}} {{n-k+1} \choose {\ell-\frac{k}{2}}} {{n-k+1} \choose {\ell-\frac{k-2}{2}}}$,
\begin{equation} \label{eq:quadratic-form-kikuchi-even}
(x^{\star \ell})^{\top} A x^{\star \ell} = \frac{m^2}{p} D \cdot  f(x)
\end{equation}
Further, since $x^{\star \ell}$ has $\pm 1$-valued entries, $\val(f) \leq \frac{p}{m^2 D} \boolnorm{A}$.% and $\sosval(f) \leq 1.8 \cdot \frac{\sqrt{p}}{m^{3/2}} D^{-2} \cdot \boolnorm{A}$.
\end{lemma}

\begin{proof}
To see \eqref{eq:quadratic-form-kikuchi}, observe that by definition of $A$, every pair $(C,C') \in \cH_u \times \cH_u$, $C \neq C'$ appears exactly ${{k-1} \choose \frac{k}{2}} {{k-1} \choose \frac{k-2}{2}} {{n-k+1} \choose {\ell-\frac{k}{2}}} { {n-k+1} \choose {\ell-\frac{k-2}{2}}} = D$ times when we expand the LHS. The equation immediately follows. The ``further...'' now follows by the definition of the $\infty \rightarrow 1$-norm.
\end{proof}



In order to implement row pruning, let's define \emph{large} rows/columns of $A$. 

\begin{definition}[$\Bad$ Rows in \kikuchi matrix]
\label{def:badrows}
Let $\Delta = \Gamma \log^{3k} (n)$ for some large enough constant $\Gamma>4k$. For any $S \in {{[n]} \choose \ell}$, let $\deg_{u,L}(S) = |\{ C \in \cH_u \mid |S \cap C| = \frac{k}{2}\}|$. Similarly, let $\deg_{u,R}(S) = |\{ C \in \cH_u \mid |S \cap C| = \frac{k-2}{2}\}|$. We say that a row indexed by $(S_1,S_2) \in {{[n]} \choose \ell}$ is \emph{bad} if for some $u \leq p$, $\deg_{u,L}(S_1) \deg_{u,R}(S_2)> d$.\peter{should be $\Delta$?} We let $\cB$ be the set of bad rows in $A$. 
% For $C \subseteq [n]$, and $u \in [p]$, let $\deg_u(C)$ be the number of $C' \subseteq [n]$, such that $C' \cap C = \emptyset$ and $C \cup C' \in \cH_u$. For $S \subseteq [n]$, $\abs{S} = \ell$, let $\deg_u(S) = \sum_{C \subseteq S : \abs{C} = \frac{k}{2}} \deg_u(C)$.
% Let $d = O(\log n/\eps)$. We define $\Bad$ to be the set of $S$ such that $\deg_u(S) > d$ for some $u \in [p]$; a row/column $(S_1, S_2)$ in the \kikuchi matrix $A$ is \emph{bad} if at least one of $S_1,S_2$ is in $\Bad$. We let $\cB$ denote the set of bad rows/columns of $A$.
\end{definition} \pravesh{$\Delta$ defined in the first line, right?}

We bound the number of bad rows in the following lemma.
\begin{lemma}[Bounding $|\cB|$]
\label{lem:numbadrows-even}
Let $\cB$ be the set of bad rows (Definition~\ref{def:badrows}) in \kikuchi matrix $A$ for the polynomial $f$ in \eqref{eq:poly-after-C-S}. Then, $|\cB| \leq N^2/n^{\Gamma} \leq \frac{N^2}{n^{3k}}$.
\end{lemma} 
\peter{typo above?, should be $n^{\Delta}$? or else $2^{\Delta}$?} \pravesh{I think it should be $1/n^{\Gamma}$ if I applied Schudy correctly.}



With the above bound on the fraction of large rows, we are ready to implement the row pruning step. 

\begin{lemma}[Row Pruning]
\label{lem:row-pruning-even}
Let $k \in \N$ be even. Let $A$ be the \kikuchi matrix defined in~\eqref{eq:kikuchi-matrix-def} for a regular, partitioned homogenous multilinear degree $k$ polynomial $\psi$ described by $\{\cH_u\}_{u \leq p}$ and coefficients $\{b_{u,C}\}_{C \in \cH_u, u \leq p}$.
Let $\cG$ be the set of $(S_1,S_2) \notin \cB$ be the good rows of $A$. Let $A_{\cG, \cG}$ be the matrix obtained by zeroing out rows and columns in $\cB$. %Recall that $D={{k-1} \choose \frac{k-1}{2}} {{n-k+1} \choose {\ell-\frac{k-1}{2}}}$. 

Then (regardless of the coefficients $\{b_{u,C}\}_{C \in \cH_u}$s),  
\[
\frac{p}{m^2} \frac{1}{D} \boolnorm{A-A_{\cG,\cG}} \leq \frac{3}{n} \mper    %O\Paren{\frac{\eps^2 N^2 m^2}{n^{40k}}}\mper
\] % and $\boolnorm{M} \leq O(\frac{\eps^2 N^2 m^2}{n^{40k}})$.
\end{lemma}

\begin{proof}

Let $A_{\cB,\cB}$ be the matrix obtained by zeroiing out row and columns not in $\cB$.
Let $A_{\cG,\cB}$ ($A_{\cB,\cG}$, respectively) be the matrix obtained by zeroing out rows (columns, respectively) in $\cB$. 

Then, note that $A-A_{\cG,\cG} = A_{\cG, \cB} + A_{\cB, \cG} + A_{\cB, \cB}$. Let's first obtain a loose upper-bound on the spectral norm of th each of the three term above by upper-bounding the maximum $\ell_1$ norm of any of their rows. The non-zero entries in any row $(S_1, S_2)$ of $A$ (and therefore also any of the three terms on the RHS above) corresponds to pairs $(T_1, T_2)$ such that $S_1 \overset{C}{\leftrightarrow} T_1$ and $S_2 \overset{C'}{\leftrightarrow} T_2$ for some pair of constraints $C,C' \in \cH_u$ for some $u \in [p]$. Each pair $(T_1, T_2)$ determines $C,C'$ so any given pair $(C,C')$ can appear at most once in any row. Further, $b_{u,C} \in [-1,1]$ for every $C$. We thus immediately obtain an upper-bound of $\sum_{u\in [p]} |\cH_u|^2 \leq p\frac{m^2}{p^2} \leq m^2 \leq n^{2k}$ on the $\ell_1$ norm of any row. 

We now observe that for any $Y,Z \in \on^N$, $Y^{\top} A_{\cG, \cB} Z \leq |\cG|^{1/2} |\cB|^{1/2} \Norm{A_{\cG,\cB}}_2 \leq n^{2k} \cdot (N^2)^{1/2} \cdot \frac{(N^2)^{1/2}}{n^{\Gamma}} \leq \frac{1}{n}$ whenever $\Gamma>2k+1$. Similarly, $Y^{\top} A_{\cB, \cG}Z \leq \frac{1}{n}$ when $\Gamma>2k$. 

Finally, $Y^{\top} A_{\cB,\cB} Z \leq |\cB| \cdot n^{2k} \leq N^2 \cdot \frac{1}{n^{2k}}$ whenever $\Gamma >2k$. This completes the proof.


% Let's obtain a loose upper-bound on $\Norm{A'}_{2}$ by noting that it is at most $\max_{S_1, S_2 \in {{[n]} \choose \ell}} \Norm{A((S_1,S_2), ;)}_1$ -- the maximum $\ell_1$-norm of any row of $A'$. 



% Let $\alpha = \frac{\abs{\Bad}}{N}$. By \cref{lem:numbadrows}, we have $\alpha \leq O(\eps^4 n^{-99})$.
% We observe that for any pair $(S_1, S_2)$, we must have $\sum_u \deg_u(S_1) \deg_u(S_2) \leq \gamma(S_1, S_2) \cdot \max_u \abs{\cH_u} \leq m^2$. Hence, the $\ell_1$ norm of any row/column in either of $B$ or $M$ is at most $m^2$. Hence, $\norm{B}, \norm{M} \leq m^2$. It then follows that $\boolnorm{B} \leq \abs{\cB} \norm{B} \leq \alpha N^2 \cdot m^2$ and $\boolnorm{M} \leq \sqrt{\abs{\cG} \abs{\cB}} \norm{M} \leq \sqrt{\alpha} N^2 \cdot m^2$. As $\alpha \leq O(\eps^4 n^{-99})$, we have the desired bound on $\boolnorm{B}$ and $\boolnorm{M}$.
\end{proof}

We finally come to the technical heart of the proof that bounds $\boolnorm{A_{\cG,\cG}}$.
\begin{lemma}\label{lem:bool-norm}
Let $A$ be the \kikuchi matrix defined in~\eqref{eq:kikuchi-matrix-def}.
Let $\cG$ be the set of $(S_1,S_2) \notin \cB$ be the good rows of $A$. 
Then, with probability at least $1-o_n(1)$ over the draw of the coefficients $\{b_{u,C}\}_{C \in \cH_u, u\in [p]}$ from independent mean $0$ distributions on $[-1,1]$, $\boolnorm{A_{\cG, \cG}} \leq O(\log m) {n \choose \ell} m \sqrt{\frac{D}{P}} \sqrt{\ell} \sqrt{ \log n}$. Here, recall that $D = {{k-1} \choose \frac{k}{2}} {{k-1} \choose \frac{k-2}{2}} {{n-k+1} \choose {\ell-\frac{k}{2}}} {{n-k+1} \choose {\ell-\frac{k-2}{2}}}$.
\end{lemma}


We can finish the proof of~\cref{thm:partitioned-poly-refute-even} immediately now:
\begin{proof}

From ~\cref{lem:cauchy-schwarz-trick-even}, we know that:
\[
\val(f) \leq \frac{p}{m^2 D} \boolnorm{A}\mper
\]
From ~\cref{lem:bool-norm}, with probability at least $1-o(1)$, we know that $\boolnorm{A_{\cG, \cG}} \leq O(\log m) {n \choose \ell} m \sqrt{\frac{D}{p}} \sqrt{\ell} \sqrt{ \log n}$. Combined with Lemma~\ref{lem:row-pruning-even}, we obtain an upper-bound on $\boolnorm{A}$. Plugging into Lemma~\ref{lem:cauchy-schwarz-trick-even} gives an upper-bound on $\val(f)$, which, immediately yields an upper-bound of $\epsilon^2$ on $\val(\psi)^2$ as desired.



\end{proof}

\subsection{Bounding Bad Rows: Proof of \cref{lem:numbadrows-even}}


\begin{proof}[Proof of \cref{lem:numbadrows-even}]
In order to bound the number of bad rows, we will analyze the probability that a uniformly random $S \in {{[n]} \choose \ell}$ is a bad set of size $\ell$. Then, observe that: %For each $i \leq (k-1)$, let $S^{(i)} = \cup_{j \leq \ell} S_{i,j} \subseteq [n]$. Then, observe that 
\[
 \deg_{u,L}(S) = \sum_{C \in \cH_u} \sum_{R \subseteq C, |R| = \frac{k}{2}} \1(S \cap C = R) \leq  \sum_{C \in \cH_u} \sum_{R \subseteq C, |R| = \frac{k}{2}} \1(S \supseteq R) \mcom
\]
\[
 \deg_{u,R}(S) = \sum_{C \in \cH_u} \sum_{R \subseteq C, |R| = \frac{k-2}{2}} \1(S \cap C = R) \leq  \sum_{C \in \cH_u} \sum_{R \subseteq C, |R| = \frac{k-2}{2}} \1(S \supseteq R) \mcom
\]

Observe that the upper bounds on the RHS above are polynomials in the $0$-$1$ indicator of the input set $S$ of degree $\frac{k}{2}$ and $\frac{k-2}{2}$, respectively that we explicitly write down below:
\begin{equation} \label{eq:poly-for-degus-left}
P_{u,L}(z) := \sum_{C \in \cH_u} \sum_{R\subseteq C, |R| = \frac{k}{2}} z_R \mcom
\end{equation} 
\begin{equation} \label{eq:poly-for-degus-left}
P_{u,R}(z) := \sum_{C \in \cH_u} \sum_{R\subseteq C, |R| = \frac{k-2}{2}} z_R \mper
\end{equation} 
Here, $z_R = \prod_{r \in R} z_r$ for every $r$.

Since $P_{u,L}(z)$ ($P_{u,R}(z)$, respectively) upper bounds $\deg_{u,L}(S)$ ($\deg_{u,R}(S)$, respectively), it's enough to upper-bound the upper-tail of $P_{u,L}(z)$ ($P_{u,R}(z)$, respectively). We will do this by relating the behavior of $P_{u,L}(z)$ and $P_{u,R}(z)$ on the $0$-$1$ indicator of a random set of size $\ell$ to a closely related product distribution.  

\begin{claim}[Reduction to Product Measure]
Let $\mu^{n}$ be the distribution of $z \in \zo^n$ where each coordinate $z_i$ is an independent random variable with $\Pr[z_i = 1] = \frac{\ell}{n} \cdot \log^2(n)$.

Then, for any $\lambda$, 
\[
\Pr_{S \sim {{[n]} \choose \ell}}[\deg_{u,a}(S) > \lambda] \leq \Pr_{z \sim \mu^{n}}[ P_{u,a}(z) > \lambda] + n^{-\log n} \mcom
\]
for $a \in \{L,R\}$.

\end{claim}
\begin{proof}[Proof of Claim]
Note that under $\mu^{n}$, each $z$ can indicate a set of size not equal to $\ell$ unlike in the distribution of $z$ obtained by choosing a uniform $S \sim {{[n]} \choose \ell}$ as described above. In order to relate the behavior of $P_{u,a}(z)$ on $\mu^n$ to that on uniform uniform $S \sim {{[n]} \choose \ell}$, we will couple the two distributions as follows: 

if $z \sim \mu^n$ is the indicator of a set $T$ of size $\geq \ell$, then let $S$ be a uniformly random subset of size $\ell$ of $T$. Otherwise abort. Observe that this coupling succeeds whenever each $T$ has at least $1$ element. By Chernoff bound, $\Pr[ |T| \geq \ell] \leq n^{-\log n}$. Further, notice that if the coupling succeeds and outputs $(T,S)$, then $P_{u,a}(T) \geq \deg_u(S)$. We thus have:
\[
\frac{\Pr_{(T,S)} [P_{u,a}(z) > \lambda ]}{\Pr[ \text{ coupling succeeds }]} \geq \Pr[ \deg_{u,a}(S) > \lambda]\mper
\]

The lemma now follows by observing that $\frac{1}{1-\alpha} \leq 1+ \alpha$ for any $\alpha <1/2$.
\end{proof}

Let's now compute the average of $P_{u,L}(z)$ when $z$ is chosen from $\mu^{n}$. For any $C \in \cH_u$ and $R \subseteq C$, observe that $\E_z z_R = \Paren{\sqrt{\frac{\ell}{n}}}^{|R|} \log^{2k-2}(n)$. \peter{shouldnt it be $\log^{2 \abs{R}} n$?} \pravesh{yes} Thus, 
\[
\E P_{u,L}(z) \leq |\cH_u| \cdot \Paren{\frac{\ell}{n}}^{\frac{k}{2}} \log^{2k-2}(n) \leq \frac{\ell}{n}  \log^{2k-2}(n)\mcom
\] for every $\ell\leq n$. 
Similarly, 
\[
\E P_{u,R}(z) \leq |\cH_u| \cdot \Paren{\frac{\ell}{n}}^{\frac{k}{2}-1} \log^{2k-2}(n) \leq \log^{2k-2}(n)\mcom
\]


We apply the the Schudy-Sviridenko inequality~\cref{fact:schudy-sviridenko} first to the polynomial $P_{u,L}(z)$. 
From \eqref{eq:poly-for-degus}, $P_{u,L}$ is clearly a sum of ${{k-1} \choose {\frac{k}{2}}} \cdot |\cH_u|$ monomials of degree exactly $\frac{k}{2}$. Observe that the collection of monomials $H$ for $P_{u,L}(z)$ equals $\{R \mid |R| = \frac{k}{2}, R \subseteq C, C \in \cH_u\}$. 

Let's now compute $\nu_r$. Since $\{\cH_u\}_{u \leq p}$ is regular at $\ell$, we know that $|\cH_{u,R}|\leq \frac{1}{\epsilon^4} 2m/p \Paren{\frac{\ell}{n}}^{r}$ for every $r \leq \frac{k-2}{2}$. For $r = \frac{k-2}{2}$, this bound is at most $O(\frac{1}{\epsilon^4})$. Thus, we immediately also obtain that $|\cH_{u,R}| \leq O(\frac{1}{\epsilon^4})$ for $|R| = \frac{k}{2}$.
Thus, for $r = \frac{k-2}{2}$, 
\[
\nu_r \leq \frac{1}{\epsilon^4} 2m/p \Paren{\frac{\ell}{n}}^{r} \cdot \Paren{\frac{\ell}{n}}^{\frac{k}{2}-r} \leq  \frac{\ell}{n} \log^{k-1}(n) \leq \frac{\log^{k-1}(n)}{\epsilon^4} \mcom
\] 
\peter{the $2m/p$ appears twice. typo?}
where in the last inequality we used that $\ell \leq n$. Note that this last inequality is \emph{not} tight for $\ell \ll n$. 
And for $r = \frac{k}{2}$, we have:
\[
\nu_r \leq \frac{1}{\epsilon^4} \leq  \frac{1}{\epsilon^4} \leq \frac{\log^{k-1}(n)}{\epsilon^4}\mcom
\] 

% Let's now compute $\nu_r$ for larger $r = 1$ (we do this to demonstrate the smallest $r$ for which our regularity parameters are optimal). By regularity of $\cH$, for any choice $v$, $|\cH_{u,\{v\}}|\leq |\cH_u| \cdot \sqrt{\frac{\ell}{n}}$. Thus, 
% \[
% \nu_r \leq \frac{m}{p} \sqrt{\frac{\ell}{n}} \Paren{\frac{\ell}{n}}^{\frac{k-1}{2}-1} \leq \log^{2k-4}(n)\mper
% \] Unlike the previous case, observe that this last inequality is tight.

% Finally, let's compute $\nu_r$ for $2 \leq r \leq \frac{k-1}{2}$ which is similar to above. By regularity of $\cH$ again, for any $R$ of size $|R|\geq 2$, it must hold that $\deg_u(R)\leq |\cH_u| \cdot \sqrt{ \frac{\ell}{n}} \Paren{\frac{\ell}{n}}^{r-2}$. Thus, 
% \[
% \nu_r \leq \frac{m}{p} \sqrt{ \frac{\ell}{n}} \Paren{\frac{\ell}{n}}^{r-1} \Paren{\frac{\ell}{n}}^{\frac{k-1}{2} -r} \leq \log^{2k-2r}(n)\mper
% \] Here again, the last inequality is tight as in the previous case 

Applying the Schudy-Sviridenko inequality now immediately completes the proof. %Notice that for every $r \leq k/2$, $\nu_r$ is clearly upper-bounded by $|\cH_u| \cdot \mu^{k/2-r}$.  

Let's now repeat the same calculations for $P_{u,R}(z)$. 
From \eqref{eq:poly-for-degus}, $P_{u,R}$ is clearly a sum of ${{k-1} \choose {\frac{k-2}{2}}} \cdot |\cH_u|$ monomials of degree exactly $\frac{k-2}{2}$. Observe that the collection of monomials $H$ for $P_{u,R}(z)$ equals $\{R \mid |R| = \frac{k-2}{2}, R \subseteq C, C \in \cH_u\}$. 

Let's now compute $\nu_0$. Since $\{\cH_u\}_{u \leq p}$ is regular, we know that $|\cH_{u,R}|\leq \frac{1}{\epsilon^4} 2m/p \Paren{\frac{\ell}{n}}^{r}$. 
Thus, 
\[
\nu_r \leq \frac{1}{\epsilon^4} 2m/p \Paren{\frac{\ell}{n}}^{r} \cdot \frac{1}{\epsilon^4} \Paren{\frac{\ell}{n}}^{\frac{k-2}{2}-r} \log^{k-1}(n) \leq \frac{\log^{k-1}(n)}{\epsilon^4} \mcom
\] where in the last inequality we used that $\ell \leq n$. Note that unlike in the previous calculation, this last inequality is \emph{tight}. 

Applying the Schudy-Sviridenko inequality again completes the proof.

\end{proof}

% \begin{definition}[Degrees]
% For each $S_1 \in Y_{\ell'+1,\ell'},S_2 \in {{[n]} \choose \ell}$, let 
% \[
% deg((S_1, S_2)) = \sum_{u: (1,u) \in S_1} \sum_{v \in [p]} \sum_{\substack{C \in \cH_{u,v'} \\ v' = v \mod n}} \1(|C \cap S_2| = \frac{k-2}{2})\mper
% \]
% Similarly, for each $S_1 \in Y_{\ell',\ell'+1},S_2 \in {{[n]} \choose \ell}$, let 
% \[
% deg((S_1, S_2)) = \sum_{u \in [p]} \sum_{v: (2,v) \in S_1}  \sum_{ \substack{C \in \cH_{u,v'} \\ v' =v \mod n}} \1(|C \cap S_2| = \frac{k-2}{2})\mper
% \]
% Observe the trivial upper-bound $\deg((S_1,S_2)) \leq m \frac{p}{n}$.
% \end{definition}
\begin{definition}[Butterfly Degree for Even $k$]
\label{def:butterfly-degree-even}
Let $(S_1,S_2) \in {{[n]} \choose \ell} \times {{[n]} \choose \ell}$. The butterfly-degree $\gamma(S_1,S_2)$ is defined as:
\begin{equation}
\gamma(S_1, S_2) = \sum_{u \in [p]} \deg_{u,L}(S_1) \deg_{u,R}(S_2)\mper \label{eq:butterfly-degree-even}
\end{equation}
\end{definition}

\begin{lemma}[Bounds on Butterfly Degree] \label{lem:avg-butterfly-degree}
The maximum butterfly degree of any $(S_1,S_2)$ satisfies: $\gamma(S_1,S_2) \leq m^2/p$.
The sum of the butterfly degrees satisfies:
$\sum_{(S_1,S_2) \sim {{[n]} \choose \ell} \times {{[n]} \choose \ell}} \gamma(S_1,S_2) = D|\cH_u| (|\cH_u|-1) \leq Dm^2/p$. 
\end{lemma}
\begin{proof}
Observe that 
\[
\deg_{u,L}(S_1) \deg_{u,R}(S_2) =\sum_{(C,C') \in \cH_u} |\{(C,C') \mid C \neq C', |C \cap S_1 |= \frac{k}{2}, |C' \cap S_2| = \frac{k-2}{2} \}|\mper
\] Further, observe that any given pair $(C,C')$ can contribute either $0$ or $1$ to the RHS. Thus, we immediately derive an upper-bound of $p|\cH_u|^2 \leq m^2/p$ on the maximum butterfly degree. 

Next, observe that:
\begin{align*}
\sum_{ (S_1, S_2)}  \deg_{u,L}(S_1) \deg_{u,R}(S_2) &=\sum_{(C,C') \in \cH_u} |\{(C,C') \mid C \neq C', |C \cap S_1 |= \frac{k}{2}, |C' \cap S_2| = \frac{k-2}{2} \}|\\
&= \sum_{(C,C') \in \cH_u, C \neq C'}  |\{(S_1, S_2) \mid |S_1 \cap C| = \frac{k}{2}, |C' \cap S_2| = \frac{k-2}{2}\}|\\
&= |\cH_u|(|\cH_u|-1) \cdot {{k-1} \choose {\frac{k}{2}}} {{k-1} \choose {\frac{k-2}{2}}} {{n-k+1} \choose {\ell - \frac{k}{2}}} \cdot { {n-k+1} \choose {\ell-\frac{k-2}{2}}} = D|\cH_u|(|\cH_u|-1)\mper
\end{align*}

The lemma now follows by summing over $u \in [p]$ and using the upper bound on $|\cH_u|$.


\end{proof}

\begin{definition}[Row/Column Bucketing] \label{def:row-col-bucketing-even}
Let $d_0 = \frac{Dm^2}{pN^2}$ be an upper-bound on average butterfly degree (see Lemma~\ref{lem:avg-butterfly-degree}). 
Let 
\[
R_0 = \{ (S_1, S_2) \mid \gamma(S_1,S_2) \leq d_0\}\mper
\]
For $i \geq 1$, let 
\[
R_i = \{ (S_1, S_2)  \mid 2^{i-1} d_0 < \gamma(S_1,S_2) \leq 2^{i}d_0\}\mper
\] 
% Similarly, let $R_i = \{ (T_1,T_2) \in Y_{\ell',\ell'+1} \times {{[n]} \choose \ell}  \mid 2^i d_2 < \deg((S_1,S_2)) \leq 2^{i+1}d_2\}$. 
For each $i,j \leq O(\log m)$, let $A_u^{(i,j)}$ be the matrix obtained by zeroing out rows not in $R_i$ and columns not in $R_j$ of the \kikuchi matrix $A_u$. And let $A^{(i,j)} = \sum_{u \in [p]} A_u^{(i,j)}$.
\end{definition}

\begin{lemma}[Size of Row/Column Partitions] \label{lem:size-of-partitions}
For each $i$, we have:
\[
|R_i| \leq 2^{-i+1} N^2 \mper
\]
\end{lemma}
\begin{proof}
Immediate by applying Markov's inequality to the estimate of the sum of the butterfly degrees from Lemma~\ref{lem:avg-butterfly-degree}.


\end{proof}


\begin{lemma}[Spectral Norms of $A^{(i,j)}$]
Let $A^{(i,j)}$ be the matrix defined in \cref{def:row-col-bucketing-even}. Then, with probability at least $1/n^{\ell}$,
\[
\Norm{A^{(i,j)}}_2 \leq O(1) \cdot 2^{0.5 \max\{i,j\}} \sqrt{d_0} \cdot \sqrt{\ell} \sqrt{\log n}\mper
\]
\end{lemma}

\begin{proof}
Observe that 
\[
A^{(i,j)} = \sum_{u \in [p]} A_u^{(i,j)} \mper
\]

Observe that $A_u$ are \emph{independent} random matrices (with randomness coming in only from the draw of the coefficient $b_{u,C}$s) since $b_{u,C}$s for $C$ in distinct $\cH_u$s are independent. 

We will use the rectangular matrix Bernstein inequality to upper-bound $\Norm{A^{(i,j)}}_2$. Towards this, observe that since we have zeroed out all the bad rows in each $A_{u}^{(i,j)}$ and each $b_{u,C} \in [-1,1]$, the maximum $\ell_1$ norm of any row $(S_1,S_2)$ of $A_u^{(i,j)}$ is at most $\deg_{u,L}(S_1) \deg_{u,R}(S_2) \leq \Delta^2$. Thus, by the Gershgorin circle theorem, we immediately get that $\Norm{A_u^{(i,j)}}_2 \leq \Delta^2$. 

Let us now estimate the ``variance-term'' in $A_u^{(i,j)}$. We have:
\begin{align*}
&\sum_{u \in [p]} \E A_u^{(i,j)} {A_u^{(i,j)}}^{\top} ((S_1,S_2), (T_1, T_2)) = \sum_{u \in [p]} \sum_{U_1, U_2} A_u^{(i,j)}((S_1, S_2), (U_1,U_2)) A_u^{(i,j)} ((T_1, T_2), (U_1, U_2))\\
&= \sum_{U_1, U_2}\sum_{u \in [p]} \sum_{C_1, C_1', C_2, C_2' \in \cH_u} b_{u,C_1} b_{u,C_1'} b_{u,C_2}b_{u,C_2'} \1( S_1 \overset{C_1}{\to} U_1) \1( S_2 \overset{C_1'}{\to} U_2) \1( T_1 \overset{C_2}{\to} U_1) \1( T_2 \overset{C_2'}{\to} U_2)\mper
\end{align*}

Observe that by independence of $b_C$'s for $C \in \cH_u$, the expectation of any given term (corresponding to $(C_1, C_1', C_2, C_2')$) is non-zero only when $C_1 = C_2, C_1' = C_2'$ (recall that $C_1 \neq C_1'$, $C_2 \neq C_2'$ in any non-zero entry).\peter{why cant we have $C_1 = C'_2, C_2 = C'_1$?} \pravesh{intersection sizes are different.}
When non-zero, this expectation is non-negative and at most $1$ since $b_C \in [-1,1]$ for all $C$. This implies that $((S_1, S_2), (T_1,T_2))$ entry above is non-zero when $S_1 = T_1, S_2 = T_2$. Further, the $((S_1,S_2), (S_1,S_2))$ diagonal entry above is at most the number of pairs $(C_1,C_1')$ above which is exactly $\gamma(S_1,S_2))\leq 2^i d_0$. This immediately yields that:
\[
\Norm{\sum_{u \in [p]} \E A_u^{(i,j)} {A_u^{(i,j)}}^{\top}}_2 \leq 2^i d_0\mper
\]

By a similar argument, we get that:
\[
\Norm{\sum_{u \in [p]} \E {A_u^{(i,j)}}^{\top} {A_u^{(i,j)}}}_2 \leq 2^j d_0\mper
\]

We now apply the matrix Bernstein inequality to conclude that: 
\[
\Norm{A^{(i,j)}}_2 \leq O(1) \cdot 2^{0.5 \max\{i,j\}} \sqrt{d_0} \cdot \sqrt{ \log N^2 }\mper
\]
This completes the proof. 

\end{proof}

\begin{proof}[Proof of Lemma \ref{lem:bool-norm}]

Observe that:
\[
A = \sum_{i,j} A^{(i,j)}\mper
\]

From Lemma~\ref{lem:size-of-partitions}, we know that number of non-zero rows (columns, respectively) in $A^{(i,j)}$ are at most $2^{-i+1} N^2$ ($2^{-j+1} N^2$, respectively).

Thus, for any vectors $Y, Z\in \on^{N^2}$, we must have:

\[
Y^{\top} A Z \leq \sum_{i,j \leq O(\log m)} \sqrt{|R_i|} \sqrt{|R_j|} \cdot \Norm{A^{(i,j)}}_2 \mper
\]
Each term indexed by $i,j$ on the RHS contributes at most $2^{-(i+j)/2} N^2 \max\{ 2^{i/2}, 2^{j/2}\} \cdot \sqrt{d_0 \ell} \sqrt{\log n}$. Thus, in total the sum is at most $O(\log m) N^2 \sqrt{d_0 \ell} \sqrt{ \log n}$.

\end{proof}









% The following lemma is immediate:

% \begin{lemma}[Decoupling]
% Let $p$-heavy (for $p= nt$ for some integer $t$) partitioned homogenous degree $k$ polynomial $\psi(y,x)$ be specified by $\{\cH_u\}_{u \in [p]}$ and $\{b_{C}\}_{C\in \cH_u, u \in [p]}$:
% \[
% \psi(y,x) = \sum_{u \leq p} y_u \sum_{C \in \cH_u} b_{u,C} x_C \mper
% \]
% For $v \in [n]$, let $\cH_{u,v} = \{ C \mid C \cup \{v\} \in \cH_u, v<C_{min}\}$ where for any subset $C \subseteq [n]$, we define $C_{min}$ to be the minimum element in it. Let
% \begin{equation} \label{eq:decoupled}
% \psi'(y^{(1)}, y^{(2)}, x) = \sum_{u \in [p], v \in [n]} y^{(1)}_u y^{(2)}_v \sum_{C \in \cH_{u,v}} b_{v,C} x_C\mper
% \end{equation}
% Then, $\max_{y,x} \psi(y,x) \leq \max_{y^{(1)}, y^{(2)}, x} \psi'(y^{(1)}, y^{(2)}, x)$.
% \end{lemma}

% We will now exclusively focus on refuting $\psi'$ defined in \eqref{eq:decoupled}. As in the previous section, we will do this by writing $\psi'$ as a quadratic form of an appropriate variant of \kikuchi matrix defined below. 

% \begin{definition}[\kikuchi matrix for even $k$]
% Let $\ell = \ell(n) = 2\ell'+1$ be an even positive integer. 
% Let $Y^{(1)} = \{ (1,i) \mid i \leq p\}$ be a universe corresponding to the coordinates of $y^{(1)}$.
% Let $Y^{(2)} = \{ (2,j) \mid j \leq p \}$ be a universe corresponding corresponding to the coordinates of $y^{(2)}$ where we assocaite every $j \leq p = nt$ to the coordinate $j \mod p$.

% Let $N_1 = 2{p \choose {\ell'+1}}{p \choose {\ell'}}$. 
% Let $N_2 = {n \choose \ell}$. 


% Let $S_1 \subseteq Y^{(1)} \cup Y^{(2)}$ be a set of size $\ell = 2 \ell'+1$ such that $|S_1 \cap Y^{(1)}| = \ell'+1$ and $|S_1 \cap Y^{(2)}| = \ell'$. Call the set of all such sets as $Y_{\ell'+1,\ell'}$. 

% Let $T_1 \subseteq Y^{(1)} \cup Y^{(2)}$ be a set of size $\ell = 2 \ell'+1$ such that $|S_1 \cap Y^{(1)}| = \ell'$ and $|S_1 \cap Y^{(2)}| = \ell'$. Call the set of all such sets as $Y_{\ell',\ell'+1}$. 

% Let $S_2, T_2 \subseteq [n]$ be subsets of size exactly $\ell$. 

% For every $u,v$, let:
% \[
% A_C((S_1, S_2), (T_1, T_2)) =  b_{v,C} \cdot \1 (S_1 \overset{u,v}{\leftrightarrow} T_1) \1(S_2 \overset{C}{\leftrightarrow} T_2)\mcom
% \]
% where we say that $S_1 \overset{u,v}{\leftrightarrow} T_1$ if the symmetric difference $S_1 \Delta T_1 = \{ (1,u), (2,v')\}$ for $v' = v \mod n$ and $S_2 \overset{C}{\leftrightarrow} T_2$ if the symmetric difference $S_2 \Delta T_2 = C$ and use the convention that $b_{v,C} = 0$ whenever $C \not \in \cH_{u,v}$. Set all the other entries to $0$.

% Finally, we set $A = \sum_{u,v} \sum_{C \in \cH_{u,v}} A_C$. Note that each $A_C$ and thus $A$ is a square matrix of dimensions $N \times N$ for $N = N_1 N_2$. 
% \end{definition}

% We have the following observation that immediately follows from the definition of the \kikuchi matrix above. 

% \begin{lemma}[$|\psi'$ is quadratic form of \kikuchi matrix]
% Let $\psi'$ be the polynomial defined in \eqref{eq:decoupled} specified by $\{\cH_{u,v}\}_{u \in [p], v\in [n]}$. 
% Let $D_1 = \frac{p}{n} {p \choose \ell'}^2$ and $D_2 = {{k-2} \choose {\frac{k-2}{2}}} \cdot {n \choose {\ell - \frac{k-2}{2}}}$ and $D = D_1 D_2$.
% Let $y^{\star \ell}$ be the vector with coordinates indexed distinct subsets of size $\ell$ of $Y^{(1)} \cup Y^{(2)}$.
% Let $x^{\star \ell}$ be the vector with coordinates indexed by distinct subsets of size $\ell$ of $[n]$.
% Then, 
% \[
% Dm \psi'(y^{(1)}, y^{(2)}, x) = (y^{\star \ell} \otimes x^{\star \ell})^{\top} A (y^{\star \ell}  \otimes x^{\star \ell})\mper
% \]
% \end{lemma}

% \begin{proof}
% Observe the the number of non-zero entry in $A_C$ for $C \in \cH_{u,v}$ equals the number of pairs $(S_1, S_2)$ and $(T_1, T_2)$ such that $S_1 \Delta S_2 = \{ (1,u), (2,v')\}$ for some $v' = v \mod n$ and $T_1 \Delta T_2 = C$. The number of pairs of the first kind are at most $D_1$ and the number of pairs of the second kind are at most $D_2$. Thus, every monomial in $\psi'$ appears in the quadratic form on the RHS exactly $D = D_1 \cdot D_2$ times. 
% \end{proof}

% As in the previous section, our proof involves establishing an upper-bound on $\boolnorm{A}$ by a careful bucketing of rows and columns of $A$. We introduce some setup and notation in the following definitions before proceeding with the argument. 

% \begin{definition}[Degrees]
% For each $S_1 \in Y_{\ell'+1,\ell'},S_2 \in {{[n]} \choose \ell}$, let 
% \[
% deg((S_1, S_2)) = \sum_{u: (1,u) \in S_1} \sum_{v \in [p]} \sum_{\substack{C \in \cH_{u,v'} \\ v' = v \mod n}} \1(|C \cap S_2| = \frac{k-2}{2})\mper
% \]
% Similarly, for each $S_1 \in Y_{\ell',\ell'+1},S_2 \in {{[n]} \choose \ell}$, let 
% \[
% deg((S_1, S_2)) = \sum_{u \in [p]} \sum_{v: (2,v) \in S_1}  \sum_{ \substack{C \in \cH_{u,v'} \\ v' =v \mod n}} \1(|C \cap S_2| = \frac{k-2}{2})\mper
% \]
% Observe the trivial upper-bound $\deg((S_1,S_2)) \leq m \frac{p}{n}$.
% \end{definition}





% \begin{definition}[Row/Column Bucketing] \label{def:row-col-bucketing}
% Let $d_0 = \frac{Dm}{N_1 N_2}$. 
% Let $R_0 = \{ (S_1, S_2) \mid \deg((S_1, S_2)) \leq d_0\}$.
% For $i \geq 1$, let $R_i = \{ (S_1, S_2)  \mid 2^{i-1} d_0 < \deg((S_1,S_2)) \leq 2^{i}d_0\}$. 
% % Similarly, let $R_i = \{ (T_1,T_2) \in Y_{\ell',\ell'+1} \times {{[n]} \choose \ell}  \mid 2^i d_2 < \deg((S_1,S_2)) \leq 2^{i+1}d_2\}$. 
% For each $i,j \leq O(\log m)$, let $A^{(i,j)}$ be the matrix obtained by zeroing out rows not in $R_i$ and columns not in $R_j$ of the \kikuchi matrix $A$.
% \end{definition}



% \begin{lemma}[Spectral Norms of $A^{(i,j)}$]
% Let $A^{(i,j)}$ be the matrix defined in Definition~\ref{def:row-col-bucketing}. Then, 
% \[
% \Norm{A^{(i,j)}}_2 \leq \mper
% \]

% \end{lemma}

% \begin{proof}
% Observe that 
% \[
% A^{(i,j)} = \sum_{u,v} \sum_{C \in \cH_{u,v}} A_C^{(i,j)} \mper
% \]
% Observe further that $A_C$s are independent random matrices (notice that the randomness here comes only from the draw of the $b_{v,C}$s). 

% We will upper-bound the spectral norm of $A^{(i,j)}$ using the matrix rectangular Bernstein inequality. Towards this, observe that each row of $A_C$ has at most $1$ non-zero entry whose magnitude is at most $1$ (since $b_{u,C} \in [-1,1]$). Thus, with probability $1$, $\Norm{A_C}_2 \leq 1$ for every $u,v, C \in \cH_{u,v}$.

% Let's now compute $\Norm{\E\sum_{u,v,C \in \cH_{u,v}} A_C A_C^{\top}}_2$. 

% For any $((S_1,S_2), (T_1, T_2))$, observe that 
% \[
% \E\sum_{u,v,C \in \cH_{u,v}} A_C A_C^{\top} ((S_1,S_2), (T_1, T_2))) = \sum_{U_1,U_2} \E A_C((S_1,S_2), (U_1, U_2)) A_C((T_1,T_2), (U_1, U_2)) \mper
% \]

% Observe that if $(T_1, T_2) \neq (S_1, S_2)$, then at most one of $A_C((S_1,S_2), (U_1, U_2))$ and $A_C((T_1,T_2), (U_1, U_2))$ can be non-zero. Thus, $(T_1, T_2) = (S_1, S_2)$ in every non-zero entry of $\E A_C A_C^{\top}$ (i.e., this matrix is diagonal). Let's now compute the maximum diagonal entry of this matrix. 

% Summing up the equation above, we see that the diagonal entry at $(S_1, S_2)$ equals $\deg((S_1, S_2)) \leq d_1 2^{i+1}$. This yields that $\Norm{\E\sum_{u,v,C \in \cH_{u,v}} A_C A_C^{\top}}_2 \leq d_1 2^{i+1}$. 

% By a similar argument, $\Norm{\E\sum_{u,v,C \in \cH_{u,v}} A_C^{\top} A_C}_2 \leq d_0 2^{j+1}$. 

% Applying the matrix Bernstein inequality now yields that:








% \end{proof}





% \section{Subexponential refutation for even $k$-XOR}
% Let $k$ be even. For $r = 1, \dots, m$, let $C_r \in {[n] \choose k}$ be distinct sets. (Note that this implies that $m \leq n^k$.) Let $b_{C_r}$ be independent real-valued random variables with $\E[b_{C_r}] = 0$, $\E[b_{C_r}^2] \leq 1$, and $b_{C_r} \in [-b,b]$ always. Let $\phi(x) := \frac{1}{m} \sum_{r = 1}^m b_{C_r} \prod_{i \in C_r} x_i$. We wish to use SoS to refute that $\max_{x \in \Fits^n} \phi(x) \leq O(\eps)$ with high probability.
% \begin{theorem}[Semirandom/smoothed sub-exponential refutation for even $k$-XOR]
% Fix $\ell \in \N$. Let $N = {n \choose \ell}$, and let $D = {k \choose k/2} \cdot {{n - k} \choose \ell - k/2}$. Suppose that $m \gg \frac{N \log N \log n}{D \eps^2}$. Let $\pE$ be a degree-$2\ell$ pseudo-expectation in $x$ over $\Fits^n$. Then with high probability over the choice of the $b_{C_r}$'s, $\pE[\phi(x)] \leq O(\eps)$.
% \end{theorem}
% We note that $\frac{N \log N}{D} \approx \frac{{n \choose \ell} \cdot \ell}{{{n - k} \choose \ell - k/2}} \approx \frac{n^{k/2}}{\ell^{k/2}} \cdot \ell$. When $\ell = n^{\delta}$, this shows that it suffices to have $m \gg n \cdot n^{(k/2 - 1)(1 - \delta)} \cdot \frac{\log^2 n}{\eps^2}$, which is what we wanted.



% Define the Kikuchi matrix $A \in \R^{N \times N}$ as $A(S,T) = b_{C_r}$ if $S \oplus T = C_r$ for some $r$ and $0$ otherwise.
% \begin{claim}
% For any $C_r$, there are exactly $D$ ordered pairs of sets $(S,T)$ such that $S \oplus T = C_r$.
% \end{claim}
% \begin{proof}
% We can specify a pair uniquely by determining the first set $S$. In order for $S \oplus T$ to be equal to $C_r$, it must be the case that $\abs{S \cap C_r} = \abs{T \cap C_r} = k/2$. It follows that we can specify $S$ by choosing $k/2$ elements from $C_r$, and then $\ell - k/2$ elements from $[n] \setminus C_r$, so we are done.
% \end{proof}

% \begin{claim}
% Fix $x \in \Fits^n$, and let $y \in \Fits^N$ be defined as $y_S := \prod_{i \in S} x_i = x_S$ for each $S$. Then $y^{\top} A y = m D \phi(x)$.
% \end{claim}
% \begin{proof}
% We have that $y^{\top} A y = \sum_{S, T} y_S A(S,T) y_T = \sum_{S, T} x_{S \oplus T} = \sum_{r = 1}^m \sum_{S, T : S \oplus T = C_r} b_{C_r} x_{C_r} = m D \cdot \phi(x)$. This is because for every constraint $C_r$, there are exactly $D$ pairs of sets $(S,T)$ such that $S \oplus T = C_r$.
% \end{proof}

% \begin{lemma}[Grothendieck]
% For any degree-$2\ell$ $\pE$ over $\Fits^n$, we have $\pE[\phi(x)] \leq O(1) \frac{1}{mD} \cdot \boolnorm{A}$.
% \end{lemma}
% \begin{proof}
% Let $\pE$ be a degree-$2\ell$ pseudo-expectation over $\Fits^n$. Let $\pE'$ be a degree-$2$ pseudo-expectation over $\Fits^N$ with variables $(y_S)_{S \in [N]}$ defined by setting $\pE'[f((y_S)_{S \in [N]})] = \pE[f((\prod_{i \in S} x_i)_{S \in [N]})]$. Note that $\pE'$ is well-defined since $\pE$ is a degree-$2\ell$ pseudo-expectation over $\Fits^n$. We then have that $m D\pE[\phi(x)] = \pE'[y^{\top} A y]$. By Grothendieck's inequality, $\pE'[y^{\top} A y] \leq O(1) \boolnorm{A}$, which finishes the proof.
% \end{proof}

% So, it suffices to argue that $\frac{1}{mD} \cdot \boolnorm{A} \leq O(\eps)$.

% We make the following definition. For a set $S$, we let $\deg(S) = \abs{\{r : \abs{S \oplus C_r} = \ell\}}$. We note that $\deg(S)$ is equal to the number of $T$ such that $A(S,T) \ne 0$, and $0 \leq \deg(S) \leq m$ always holds.

% Let $d_0 = O(\eps^2 D^2 m^2/N^2 \log N)$, let $d = 2$, and let $t = O(\log m)$. Note that by the assumption on $m$, we have $d_0 \gg \log N (\log^2 n)/\eps^2 \gg \log N$. Let $\cF_0 = \{S : \deg(S) \leq d_0\}$, and for $i \in [t]$ let $\cF_i = \{S : d_0 d^{i-1} < \deg(S) \leq d_0 d^i\}$. For $0 \leq i, j \leq t$, let $A_{i,j}$ denote the matrix where $A_{i,j}(S,T) = A(S,T)$ if $S \in \cF_i$ and $T \in \cF_j$, and is $0$ otherwise. We have that $A = \sum_{i = 0}^t \sum_{j = 0}^t A_{i,j}$. This is because the $\cF_i$'s partition $S$, as $\deg(S) \leq m$ always holds. So $\boolnorm{A} \leq \sum_{0 \leq i,j \leq t} \boolnorm{A_{i,j}} \leq \sum_{0 \leq i, j\leq t} \sqrt{\abs{\cF_i} \abs{\cF_j}} \cdot \norm{A_{i,j}}$.

% \begin{claim}
% $\abs{\cF_0} \leq N$ and for all $i \in [t]$, $\abs{\cF_i} \leq \frac{mD}{d_0 d^{i-1}}$.
% \end{claim}
% \begin{proof}
% $\abs{\cF_0} \leq N$ is trivial. We also have $d_0 d^{i-1} \abs{\cF_i} \leq \sum_{S \in \cF_i} \deg(S) \leq \sum_{S} \deg(S) = mD$.
% \end{proof}


% \begin{claim}
% For all $0 \leq i,j \leq t$, $\norm{A_{i,j}} \leq O(\sqrt{d_0 d^{\max(i,j)} \log N})$.
% \end{claim}
% \begin{proof}
% Fix $i$ and $j$. For each $r \in [m]$, let $A_{i,j}^{(C_r)}$ be the matrix where $A_{i,j}^{(C_r)}(S,T) = b_{C_r}$ if $S \in \cF_i$, $T \in \cF_j$, and $S \oplus T = C_r$, and $0$ otherwise. Note that $A_{i,j} = \sum_{r = 1}^m A_{i,j}^{(C_r)}$. Because the $b_{C_r}$'s are independent with $\E[b_{C_r}] = 0$, the $A_{i,j}^{(C_r)}$'s are independent matrices with $\E[A_{i,j}] = 0$. Also, each $A_{i,j}^{(C_r)}$ is an $N \times N$ matrix, and we have that $\norm{A_{i,j}^{(C_r)}} \leq b$ always, as each row has at most $1$ nonzero entry, and all entries have magnitude at most $b$. Let $B = \sum_{r = 1}^m {A_{i,j}^{(C_r)}}^{\top} A_{i,j}^{(C_r)}$. We have that $B(S,T) = \sum_{r = 1}^m \sum_{R \in \cF_i} A_{i,j}^{(C_r)}(R,S) A_{i,j}^{(C_r)}(R, T)$. If $S \oplus R = C_r$ and $T \oplus R = C_r$, then $S \oplus T = \emptyset$, i.e., $S = T$. So, we see that $B$ is a diagonal matrix where the $(S,S)$-th diagonal entry is $\sum_{r = 1}^m \sum_{T : T \oplus S = C_r} b_{C_r}^2$ if $S \in \cF_j$, and is $0$ otherwise. As $\E[b_{C_r}^2] \leq 1$, it follows that $\E[B]$ is a diagonal matrix where the $(S,S)$-th diagonal entry is at most $\max_{S \in \cF_j} \deg(S) \leq d_0 d^{j}$, and so $\norm{\E[B]} \leq d_0 d^{j}$. Similarly, $\norm{\E[\sum_{r = 1}^m  A_{i,j}^{(C_r)} {A_{i,j}^{(C_r)}}^{\top} ]} \leq d_0 d^{i}$. We note that $\sigma^2 = d_0 d^{\max(i,j)} \geq d_0 \gg \log N$.

% We can thus apply \cref{thm:matrixbernstein} to conclude that $\norm{A_{i,j}} \leq O(\sqrt{d_0 d^{\max(i,j)} \log N})$ with probability $1 - \frac{1}{N^2} \geq 1 - \frac{1}{n^2}$. By union bound over all $O(t^2) = O(\log^2 n)$ choices for $i,j$, we thus get the desired claim.
% \end{proof}

% We now finish the proof.
% We have
% \begin{flalign*}
% &\boolnorm{A} \leq \sum_{0 \leq i, j\leq t} \sqrt{\abs{\cF_i} \abs{\cF_j}} \cdot \norm{A_{i,j}} \leq \abs{\cF_0} \norm{A_{0,0}} + 2 \sum_{j = 1}^t \sqrt{\abs{\cF_0} \abs{\cF_j}} \cdot \norm{A_{0,j}} + 2\sum_{i = 1}^{t} \sum_{j = i}^t \sqrt{\abs{\cF_i} \abs{\cF_j}} \cdot \norm{A_{i,j}} \\
% &\leq N \sqrt{d_0 \log N} + O(1)\sqrt{N} \sum_{j = 1}^t  \sqrt{ \frac{mD}{d_0 d^{j-1}} \cdot d_0 d^{j} \log N} + O(1) \sum_{i = 1}^{t} \sum_{j = i}^t \sqrt{\frac{mD}{d_0 d^{i-1}} \cdot \frac{mD}{d_0 d^{j-1}} \cdot d_0 d^j \log N} \\
% &\leq N \sqrt{d_0 \log N} + O(1)\sqrt{mD N d \log N} \cdot t + O(1) mDt \sqrt{\frac{d \log N}{d_0}} \sum_{i = 1}^{t} \frac{1}{\sqrt{ d^{i-1}}} \\
% &\leq N \sqrt{d_0 \log N} + O(1)\sqrt{mD N \log N} \cdot t + O(1) mDt \sqrt{\frac{\log N}{d_0}} \ \text{(because $d = 2$)} \\
% &= N \sqrt{d_0 \log N} \left(1 + O(t) \sqrt{\frac{mD}{N d_0}} + O(t) \frac{mD}{N d_0} \right) \enspace.
% \end{flalign*}
% We then have that 
% \begin{flalign*}
% &\frac{mDt}{N d_0} \leq O(\log n) \frac{m D}{N} \cdot \frac{N^2 \log N}{\eps^2 D^2 m^2} = O(\log n) \frac{N \log N}{\eps^2 D m} \ll O(1) \enspace,
% \end{flalign*}
% because of our assumption on $m$ (and the fact that $t = O(\log m) = O(\log n)$ since $m \leq n^k$). Thus, we conclude that $\boolnorm{A} \leq N \sqrt{d_0 \log N}$.

% Finally, we have that 
% \begin{flalign*}
% \frac{1}{mD} \cdot \boolnorm{A} \leq \frac{N}{m D} \sqrt{d_0 \log N} = O(\eps) \enspace.
% \end{flalign*}


% \begin{theorem}[Rectangular Matrix Bernstein]
% \label{thm:matrixbernstein}
% Let $X_1, \dots, X_k$ be independent random $d_1 \times d_2$ matrices with $\E[X_i] = 0$ and $\norm{X_i} \leq R$ for all $i$. Let $\sigma^2 \geq \max(\norm{\E[\sum_{i = 1}^k X_i X_i^{\top}]}, \norm{\E[\sum_{i = 1}^k X_i^{\top} X_i]})$. Then for all $t \geq 0$, $\Pr[\norm{\sum_{i = 1}^k X_i} \geq t] \leq (d_1 + d_2) \exp(\frac{-t^2/2}{\sigma^2 + R t/3})$.

% In particular, if $\sigma^2 \geq \Omega(\log(d_1 + d_2))$ and $R \leq 1$, then setting $t =  C \sigma \sqrt{\log(d_1 + d_2)}$ for a sufficiently large constant $C$ implies that
% \begin{flalign*}
% \Pr[\norm{\sum_{i = 1}^k X_i} \geq C \sigma \sqrt{\log(d_1 + d_2)}] \leq \frac{1}{(d_1 + d_2)^2} \enspace.
% \end{flalign*}
% \end{theorem}
}
